Equivariant Representation of Configuration-Dependent Friction Tensors in Langevin Heatbaths

Dynamics of coarse-grained particle systems derived via the Mori-Zwanzig projection formalism commonly take the form of a (generalized) Langevin equation with configuration-dependent friction and diffusion tensors. In this article, we introduce a class of equivariant representations of tensor-valued functions based on the Atomic Cluster Expansion (ACE) framework that allows for efficient learning of such configuration-dependent friction and diffusion tensors from data. Besides satisfying the correct equivariance properties with respect to the Euclidean group E(3), the resulting heat bath models satisfy a fluctuation-dissipation relation. Moreover, our models can be extended to include additional symmetries, such as momentum conservation, to preserve the hydrodynamic properties of the particle system. We demonstrate the capabilities of the model by constructing a model of configuration-dependent tensorial electronic friction calculated from first principles that arises during reactive molecular dynamics at metal surfaces.

==> macros-ace.tex <==
\def\ndata{N_{d}}
\def\xibf{\bm \xi}
\def\betabf{\bm \beta}
\def\deltat{h}
\def\R{R}
\def\NN{{\mathbb{N}}}
\def\RR{{\mathbb R}}
\def\Rc{\mathcal{R}}
\def\C{{\bf C}}
\def\D{{\bf D}}
\def\trans{T}
\def\pos{{\bm q}}
\def\vel{{\bm p}}
\def\Pos{{\bm Q}}
\def\Vel{{\bm P}}
\def\Force{{\bm F}}
\def\force{{\bm f}}
\def\noise{\varepsilon}
\def\Noise{\mathcal{E}}
\def\dd{{\rm d}}
\def\proj{\mathcal{P}}
\def\pproj{\mathcal{P}}
\def\oproj{\mathcal{Q}}

\def\cmom{\bm P}
\def\Gammabf{\bm \Gamma}
\def\Sigmabf{\bm \Sigma}
\def\W{\bm W}
\def\M{\bm M}
\def\I{\bm I}
\def\0{\bm 0}
\def\v{\bm v}
\def\alphabf{\bm \alpha}
\def\betabf{\bm \beta}
\def\one{\bm 1}
\def\r{\bm r}
\def\perm{{\rm P}}
\def\gammabf{\bm \gamma}
\def\possemi{\mathcal{S}}
\def\Bc{\mathcal{B}}
\def\Bcbf\bm{{\mathcal{B}}}
\def\kp{\; \widehat{\otimes}\;} % Kronecker product
\def\op{\otimes} % outer product 


==> sections/ace-basis.tex <==

In the ACE, the atomic basis $A_{z_{i},znlm}$ is defined as a projection of the neighborhood density $\rho_i^{z}$ of all atoms of chemical element $z_i$ around atom $i$ onto the one-particle basis functions $\phi_{nlm}^{z_{i}z_{j}}$
\begin{equation}
    A_{z_{i},znlm} = \left\langle\rho_{i}^{z}|\phi_{nlm}^{z_{i}z}\right\rangle = \sum_{\substack{j\\
      \forall z_j=z}} \phi_{nlm}^{z_{i}z_{j}}(r_{ji})  ,
\end{equation}
where the one-particle basis functions are summed over atoms $j$, for which $z_{j}=z$. The $z_{i},z_{j}$ are elements $z$ of central $i$ and neighboring $j$ atoms. The density $\rho_{i}^{z}$ can be described as
\begin{equation}
    \rho_{i}^{z}(\bm{r})=\sum_{\substack{j \neq i \\ \forall z_j =z}}\delta(\bm{r}-\bm{r}_{ji}) ,
\end{equation}
and the one-particle basis function can be defined as a product of a radial function $R_{nl}^{z_{i}z_{j}}$ and spherical harmonics $Y_{l}^{m}$,
\begin{equation}
    \phi_{nlm}^{z_{i}z_{j}}(\bm{r})=R_{nl}^{z_{i}z_{j}}(r)Y_{l}^{m}(\bm{\hat{r}}) .
\end{equation}
To obtain permutation-invariant basis functions, products of atomic basis functions are constructed 
\begin{equation}
    A_{z_{i}\bm{\upsilon}}=\prod^{\nu}_{t=1} A_{z_{i}\upsilon_{t}},
\end{equation}
where $\upsilon = znlm$, $\bm{\upsilon}=(\upsilon_{1},\dots,\upsilon_{\nu})$ and $\nu$ refers to correlation order, corresponding to a ($\nu$+1)-body basis function. 
Isometry invariant basis $B_{z_{i}\eta_{\nu}}$ functions are created from the non-rotationally-invariant  basis functions $A_{z_{i}\bm\upsilon}$ 
\begin{equation}
    B_{z_{i}\eta_{\nu}}=\sum_{\bm{\upsilon}} C_{\eta_{\nu}\bm{\upsilon}}A_{z_{i}\bm{\upsilon}} ,
\end{equation}
where $C_{\eta_{\nu}\bm{\upsilon}}$ are Clebsch-Gordan coefficients, and all the allowed invariant contractions of $A_{z_{i}\bm{\upsilon}}$ are enumerated by $\eta_{\nu}$.


There is a choice to be made about how the bond environment is defined and what the reference coordinates are. 



==> sections/app_cwc_optimization.tex <==
\begin{figure}
\centering
\includegraphics[width=.9\linewidth]{plots/noau/errors_opt_rmse_arch_cutoff_aceds.pdf}
\caption{\textbf{Optimization of architecture type and cutoff distance with column-wise coupled (CWC) models.} The test (dark grey circles), and training (blue triangles) RMSEs obtained using different combinations of invariant, covariant, and equivariant representations of $\Sigmabf$ with cutoff distance of 5.0~\si{\angstrom} (left side), and the convergence of EFT with respect to cutoff distance in \si{\angstrom} units, using invariant and equivariant $\Sigmabf$ (right side). Additionally, corresponding average evaluation times are included, based on 100 EFT evaluations (red stars). The maximum correlation order of 2 and corresponding polynomial degree of 5 was used in every model shown in both figures. } 
\label{fig:optimization_arch_cutoff_ac}
\end{figure}

The parameter optimization of the models that utilize culumn-wise coupling (CWC) is shown in Figs.~\ref{fig:optimization_arch_cutoff_ac}~and~\ref{fig:optimization_ord_degr_ac}. The different $\Sigmabf$ representation types, and cutoff distances, were compared as shown in Fig.~\ref{fig:optimization_arch_cutoff_ac}. Just as in the case of models based on PWC, the equivariance is the most important property, and enables the lowest EFT evaluation RMSEs (roughly 0.06~meVps\si{\angstrom}$^{-2}$), however the inclusion of equivariant matrices causes an increase in EFT evaluation times (20~ms versus 5~ms with invariant, and 10~ms with covariant matrices).
Column-wise friction models were also trained with varying cutoff distances, between 3 and 7~\si{\angstrom} (right side of Fig.~\ref{fig:optimization_arch_cutoff_ac}). In this case, again, the convergence behavior is very close to PWC case, and the cutoff converges at roughly  5~\si{\angstrom}.

\begin{figure}
\centering
\includegraphics[width=.9\linewidth]{plots/noau/errors_opt_rmse_ord_degree_aceds.pdf}
\caption{\textbf{Optimization of maximum correlation order and maximum polynomial degree with column-wise coupled (CWC) models.} The test (dark grey circles), and training (blue triangles) RMSEs were obtained for different correlation orders with polynomial degree of 5 (left side), and polynomial degrees for a correlation order of 2 (right side). Additionally, corresponding average evaluation times are included, based on 100 EFT evaluations (red stars). Cutoff distance in both plots were set at 6~\si{\angstrom}, and both invariant and equivariant $\Sigmabf$ were used in training. } 
\label{fig:optimization_ord_degr_ac}
\end{figure}
Maximum correlation order and polynomial degree were also optimized for the column-wise coupled (CWC) models, as shown in Fig.~\ref{fig:optimization_ord_degr_ac}. Here, EFT elements converge relatively quickly, with the correlation order reaching the optimal value at 2. In case of CWC models, no further improvement is visible with the correlation order of 3. 
The optimization of the corresponding maximum polynomial degrees (for correlation order of 2) is shown in Fig.~\ref{fig:optimization_ord_degr_ac}. The convergence of the maximum polynomial degree is reached at roughly 7--8 with the test RMSEs of roughly 0.055~meVps\si{\angstrom}$^{-2}$. The difference between the degrees of 7 and 10 in test RMSEs is negligible, however, the training set RMSEs decrease from roughly 0.046~meVps\si{\angstrom}$^{-2}$, to 0.037~meVps\si{\angstrom}$^{-2}$, which may suggest that higher polynomial degrees cause overfitting. 

==> sections/discussion.tex <==
% Discussion/conclusions
%%%% MENTION


% CWC - can provide a faster model
% the best accuracy was obtained with PWC
% highly efficient linear model
% which is the first model of such kind that allows exploring larger systems

We presented an equivariant representation of the Langevin heat bath, that enables modelling of configuration-dependent properties, such as friction and diffusion tensors. The new representation satisfies all the symmetries and properties of electronic friction. On the example of NO scattering at Au(111) surface, we showcased that the representation coupled with ACE provides linear models with accuracy comparable with the previous most successful NN-based methods. The convergence behavior was explored utilizing the pair-wise coupling, revealing that equivariant representation is crucial for reaching high accuracy.

Furthermore, the independent treatment of atom-wise blocks that construct electronic friction tensors can enable the exploration of the extended systems that include more than one adsorbate molecule.

==> sections/methods-ace.tex <==


%A detailed description of the construction of the ACE basis expansion can be found in \cite{}. Here, we provide a brief summary of some aspects of ACE that are relevant for the construction of the heat bath representation that we introduce in \ref{}. 

%The Atomic Cluster Expansion (ACE) provides a framework for the systematic construction of linear bases of physical features and quantities that are equivariant maps defined on atomic sites. Given an atomic configuration  $(\r_{\iota},z_{\iota})_{\iota}$, which consists of positions $\r_{i} \in \mathbb{R}^{3}$ and the corresponding chemical composition
%\[
%(z_{i} , \{(z_{j}, \r_{ij})\}_{j \in \mathcal{N}(i)} ) 
%\]

The Atomic Cluster Expansion (ACE) allows to systematically construct a linear basis for equivariant features $\mathcal{V}( (\x_{i})_{i})$ of atomic configurations where each atom $\x_{i} =(\r_{i},z_{i})$ in the configuration is characterized by its position $\r_{i}\in \mathbb{R}^{3}$ and element type $z_{i}$, such that the features correspond to an equivariant map with respect to a group $G$:
\begin{equation}\label{eq:equivariance}
\forall g \in G ~ \forall x \in \mathbb{X}: \quad g \circ \mathcal{V}(x) = \mathcal{V}(g \star x).
\end{equation}

Depending on the feature, the map $\mathcal{V} $ may satisfy different types of equivariance symmetries with respect to the rotational group $SO(3)$. For example, if $\mathcal{V}$ is the total energy $\pot$ of configurations, then $\mathcal{V}$ takes scalar values and is invariant with respect to $SO(3)$ in the following sense
\[
\forall Q \in SO(3) ~  \forall (\r_{\iota},z_{\iota})_{\iota}: \quad \mathcal{V}((\r_{\iota},z_{\iota})_{\iota}) = \mathcal{V}((Q\r_{\iota},z_{\iota})_{\iota}),
\]
which can be understood as an instance of (\ref{eq:equivariance}) with group actions specified as $Q \circ y = y$ for all $y \in \mathbb{R}, Q \in SO(3)$, and $Q \star (\r_{\iota},z_{\iota})_{\iota}= (Q\r_{\iota},z_{\iota})_{\iota}$ for all configurations $(\r_{\iota},z_{\iota})_{\iota}$ and $Q \in SO(3)$. 
If $\mathcal{V}$  is a vector-valued feature taking values in $\mathbb{R}^{3}$, then it typically will be covariant with respect to $SO(3)$, i.e.,
\[
\forall Q \in SO(3) ~  \forall (\r_{\iota},z_{\iota})_{\iota}: \quad Q\mathcal{V}((\r_{\iota},z_{\iota})_{\iota}) = \mathcal{V}((Q\r_{\iota},z_{\iota})_{\iota}),
\]
which again can be understood as an instance of (\ref{eq:equivariance}) with $Q \circ y = Qy$. Here, and throughout the remainder of this article, group elements $Q \in SO(3)$ are to be understood as rotation matrices in $\mathbb{R}^{3 \times 3}$.

%Formally, an atomic configuration can be understood as a collection (or more precisely a multi set) $\{(\r_{i},z_{i})\}_{i}$ of pairs of atomic positions $\r_{i}$ and their corresponding element types $z_{i}$. 
A physical quantity such as the potential energy of the configuration when expanded in ACE can  be written as a function 
\begin{equation}
\mathcal{V}(\{(\r_{i},z_{i})\}_{i}) = \sum_{i=1}^{N}\mathcal{V}_{\rm site}( z_{i}, R_{i} ) \end{equation}

%The atomic cluster expansion allows to systematically construct a linear basis of properties of atomic configurations. 
%An atomic cluster expansion of a property or quantity $\mathcal{V}$ that is a function of positions $R=(\r_{1},\dots,\r_{N})$ of $N$ atoms and their corresponding element types $(z_{i})_{i=1}^{N}$ is assumed to decompose as a sum 

of site-contributions $V_{\rm site}(z_{i},R_{i}),(i =1,\dots,N)$, which are functions of the {\em atomic site}  $R_{i} = \{(\r_{ij},z_{j}) : \|\r_{ij}\| < r_{{\rm cut}}\}_{j\neq i}$ and the element type $z_{i}$ of the respective center atom with index $i$.  Here, $r_{{\rm cut}} >0$ is a prescribed cut-off distance and $\r_{ij} = \r_{j}- \r_{i}$ denotes the displacement relative to the position $\r_{i}$ of the center atom. It is convention to write atomic sites as (multi-)sets to indicate that the function $V_{\rm site}(z_{i},\cdot)$ is agnostic to any ordering of atoms within the atomic site. In extension this ensures that the property 








